Cross-Platform Video Person ReID: A New Benchmark Dataset and Adaptation Approach

In this paper, we construct a large-scale benchmark dataset for Ground-to-Aerial Video-based person Re-Identification, named G2A-VReID, which comprises 185,907 images and 5,576 tracklets, featuring 2,788 distinct identities. To our knowledge, this is the first dataset for video ReID under Ground-to-Aerial scenarios. G2A-VReID dataset has the following characteristics: 1) Drastic view changes; 2) Large number of annotated identities; 3) Rich outdoor scenarios; 4) Huge difference in resolution. Additionally, we propose a new benchmark approach for cross-platform ReID by transforming the cross-platform visual alignment problem into visual-semantic alignment through vision-language model (i.e., CLIP) and applying a parameter-efficient Video Set-Level-Adapter module to adapt image-based foundation model to video ReID tasks, termed VSLA-CLIP. Besides, to further reduce the great discrepancy across the platforms, we also devise the platform-bridge prompts for efficient visual feature alignment. Extensive experiments demonstrate the superiority of the proposed method on all existing video ReID datasets and our proposed G2A-VReID dataset.

==> table/compare_with_SOTA.tex <==
% ==================================================

\begin{table*}[t]
\centering
\scriptsize
\caption{\footnotesize Comparison with state-of-the-art methods. \dag ~ represents the model initialized by the weight of CLIP\cite{CLIP} released by OpenAI, and \ddag ~ represents the model initialized by weight of ViFi-CLIP\cite{ViFi-CLIP}. We use \textbf{bold} to indicate the best results of our methods, and \underline{underlines} to highlight the best results of other methods. 
On all datasets, our method outperforms the comparisons significantly.} 
\begin{tabular}[t]{C{2.8cm}|C{1.2cm}C{1.2cm}|C{1.2cm}C{1.2cm}|C{1.2cm}|C{1.2cm}C{1.2cm}}
\toprule
\multirow{2}{*}{Method}& \multicolumn{2}{c}{MARS} & \multicolumn{2}{c}{LS-VID} & \multicolumn{1}{c}{iLIDS} & \multicolumn{2}{c}{G2A-VReID}    \\ \cline{2-8}
 & mAP & rank-1 & mAP & rank-1 & rank-1 & mAP & rank-1 \\ \midrule
GLTR\cite{GLTR} & 78.5 & 87.0 & 44.3 & 63.1 & 86 & - & - \\ 
VRSTC\cite{VRSTC} & 82.3 & 88.5 & - & - & 83.4 & - & - \\ 
AP3D\cite{AP3D} & 85.1 & 90.1 & 73.2 & 84.5 & 88.7 & 67.7 & 57.5 \\ 
STGCN\cite{STGCN} & 83.7 & 90.0 & - & - & - & - & - \\ 
MGH\cite{MGH} & 85.8 & 90.0 & - & - & 85.6 & \underline{76.7} & \underline{69.9} \\ 
MG-RAFA\cite{MG-RAFA} & 85.9 & 88.8 & - & - & 88.6 & - & - \\ 
AFA\cite{AFA} & 82.9 & 90.2 & - & - & 88.5 & - & - \\ 
TCLNet\cite{TCLNet} & 85.1 & 89.8 & 70.3 & 81.5 & 86.6 & 65.4 & 54.7 \\ 
STRF\cite{STRF} & 86.1 & 90.3 & - & - & 89.3 & - & - \\ 
GRL\cite{GRL} & 84.8 & 91.0 & - & - & 90.4 & 52.8 & 41.4 \\ 
DenseIL\cite{DenseIL} & \underline{87.0} & 90.8 & - & - & 92 & - & - \\ 
BiCnet-TKS\cite{BiCnet_TKS} & 86.0 & 90.2 & 75.1 & 84.6 & - & 63.4 & 51.7 \\ 
PSTA\cite{PSTA} & 85.8 & 91.5 & - & - & - & 64.6 & 54.5 \\ 
STMN\cite{STMN} & 84.5 & 90.5 & 69.2 & 82.1 & 91.5 & 66.7 & 56.1 \\ 
PiT\cite{PiT} & - & 90.2 & - & - & 92.1 & 76.3 & 67.7 \\ 
SINet\cite{SINet} & 86.2 & 91.0 & 79.6 & 87.4 & \underline{92.5} & 74.5 & 65.6 \\ 
LSTRL\cite{LSTRL} & 86.8 & \underline{91.6} & \underline{82.4} & \underline{89.8} & 92.2 & - & - \\ 
\midrule
FT-CLIP\ddag & 88.00 & 91.62 & 84.07 & 90.77 & 94.00 & 78.11 & 69.32 \\ \midrule
% FT-CLIP\ddag & 87.38 & \textbf{91.82} & 82.06 & 89.49 & 94.00 & 77.34 & 68.95  \\ \midrule
VSLA-CLIP\dag &88.22 & 90.91 & 84.05 & 90.54  & \textbf{95.33} & 79.14 & 71.64 \\ 
VSLA-CLIP\ddag & \textbf{88.60} & \textbf{91.82} & \textbf{85.20} &  \textbf{91.66} & \textbf{95.33}  & \textbf{79.70} & \textbf{72.55} \\ 
% & \textcolor{red}{+1.60} & \textcolor{red}{+0.32} & \textcolor{red}{+4.17} & \textcolor{red}{+3.09} & \textcolor{red}{+5.50} & \textcolor{red}{+2.99} & \textcolor{red}{+2.44}  \\ 
 \bottomrule
\end{tabular}
\vspace{-5mm}
\label{tab:compare_with_SOTA}
\end{table*}
% ==================================================

==> table/dataset_compare.tex <==
\begin{table*}[t]
\normalsize
\centering
\scriptsize
\caption{\footnotesize Comparison of G2A-VReID with other Video-ReID datasets. \textbf{CWM} denotes the camera working mode. \textbf{AD} is the average duration of each video sequence.}
\begin{tabular}[t]{C{1.6cm}|C{1.6cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.9cm}C{1.2cm}}
\toprule
Datasets & G2A-VReID & LS-VID\cite{GLTR_LS-VID} & Mars\cite{mars} & iLIDS\cite{iLIDS} & PRID-2011\cite{PRID} & 3DPeS\cite{3DPeS} \\ \midrule
identities & 2,788 & 3,772 & 1,261 & 300 & 200 & 200  \\ 
tracklets & 5,576 & 14,943 & 20,715 & 600 & 400 & 1,000   \\ 
images & 185,907 & 2,982,685 & 1,067,516 & 42,460 & 40,033 & 200,000  \\ 
AD (s) & \textbf{16.7} & 6.7 & 5.6 & 2.4 & 3.3 & 6.7  \\ 
camera & 2 & 15 & 6 & 2 & 2 & 8   \\ 
view & \textbf{ground$\mathbf{~\&~}$sky} & ground & ground & ground & ground & ground  \\ 
CWM & \textbf{moving} & fixed & fixed & fixed & fixed & fixed   \\ \midrule
\end{tabular}
\label{tab:dataset_comparison}
\end{table*}
